A Survey on Trustworthy LLM Agents: Threats and Countermeasures

With the rapid evolution of Large Language Models (LLMs), LLM-based agents and Multi-agent Systems (MAS) have significantly expanded the capabilities of LLM ecosystems. This evolution stems from empowering LLMs with additional modules such as memory, tools, environment, and even other agents. However, this advancement has also introduced more complex issues of trustworthiness, which previous research focused solely on LLMs could not cover. In this survey, we propose the TrustAgent framework, a comprehensive study on the trustworthiness of agents, characterized by modular taxonomy, multi-dimensional connotations, and technical implementation. By thoroughly investigating and summarizing newly emerged attacks, defenses, and evaluation methods for agents and MAS, we extend the concept of Trustworthy LLM to the emerging paradigm of Trustworthy Agent. In TrustAgent, we begin by deconstructing and introducing various components of the Agent and MAS. Then, we categorize their trustworthiness into intrinsic (brain, memory, and tool) and extrinsic (user, agent, and environment) aspects. Subsequently, we delineate the multifaceted meanings of trustworthiness and elaborate on the implementation techniques of existing research related to these internal and external modules. Finally, we present our insights and outlook on this domain, aiming to provide guidance for future endeavors.

==> sections/tree_template.tex <==
% 在这一节中，我们将TrustAgent完整的分类学以及引用到的所有文献都展示在树状图Figure \ref{fig:tree}中以供easy reference。
In this section, we present the complete taxonomy of TrustAgent along with all cited references in a tree diagram (Figure \ref{tree}) for easy reference.

\begin{figure*}[t]
\label{tree}
\centering
\footnotesize
\begin{forest}
    for tree={
        forked edges,
        draw,
        rounded corners,
        node options={align=center},
        s sep=2.5pt,
        calign=center,
        grow=east,
        reversed=true,
        parent anchor=east,
        child anchor=north,
        font=\footnotesize,,
      },
      where level=1{text width=100pt, fill=blue!10, text orientation=upright, rotate=90}{},
      where level=2{text width=50pt, fill=pink!30, text orientation=upright, child anchor=west}{},
      where level=3{text width=50pt, text orientation=upright, fill=yellow!30, child anchor=west}{},
      where level=4{text width=40pt, fill=cyan!20, text orientation=upright,child anchor=west}{},
      where level=5{text orientation=upright, child anchor=west}{},
[TrustAgent, fill=gray!20, rotate=90
    [Intrinsic Trustworthiness, for tree={
        answer,
        calign=child edge, calign child=(n_children()+1)/2,
        yshift=-0.2cm,
        }
        [Brain, for tree={
            answer,
            calign=child edge, calign child=(n_children()+1)/2,
            yshift=-0.2cm,
            }
            [Attack, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Jailbreak, [{Kumar et al. \cite{kumar2023certifying}, GCG \cite{zou2023universal}, IGCG \cite{jia2024improved}, AttnGCG \cite{wang2024attngcg}, MRJ-Agent \cite{wang2024mrj}, PrivAgent \cite{nie2024privagent}, Evil Geniuses \cite{tian2023evil}, PANDORA \cite{chen2024pandora}, AgentSmith \cite{gu2024agent}, Tan et al. \cite{tan2024wolf}}, answer_work, text width=250pt]]
                [Prompt Injection, [{Liu et al. \cite{liu2023prompt}, Perez et al. \cite{perez2022ignore}, Greshake et al. \cite{greshake2023not}, Liu et al. \cite{liu2024automatic}, Shi et al. \cite{shi2024optimization}, Bagdasaryan et al. \cite{bagdasaryan2023abusing}, Zhang et al. \cite{zhang2024breaking}}, answer_work, text width=200pt]]
                [Backdoor, [{Zhou et al. \cite{zhou2025survey}, Yang et al. \cite{yang2024watch}, DemonAgent \cite{zhu2025demonagent}, BLAST \cite{yu2025blast}}, answer_work, text width=220pt]]
            ]
            [Defense, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Alignment, [{Tennant et al. \cite{tennant2024moral}, Frisch et al. \cite{frisch2024llm}, Pang et al. \cite{pang2024self}, Gao et al. \cite{gao2024aligning}, Zhang et al. \cite{zhang2024large}}, answer_work, text width=150pt]]
                [Single-model Filter, [{Ayub et al. \cite{ayub2024embedding}, Kwon et al. \cite{kwon2024slm}, StruQ \cite{chen2024struq}, ShieldLM \cite{zhang2024shieldlm}, GuardAgent \cite{xiang2024guardagent}, AgentGuard \cite{chen2025agentguard}}, answer_work, text width=160pt, fill=white]]
                [Multi-Agent Collaboration, [{Du et al. \cite{du2023improving}, Kwartler et al. \cite{kwartler2024good}, AutoDefense \cite{zeng2024autodefense}}, answer_work, text width=180pt]]
            ]
            [Evaluation, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Focused Assessment, [{InjecAgent \cite{zhan2024injecagent}, AgentDojo \cite{debenedetti2025agentdojo}, DemonAgent \cite{zhu2025demonagent}, RedAgent \cite{xu2024redagent}, RiskAwareBench \cite{zhu2024riskawarebench}, RedCode \cite{guo2025redcode}}, answer_work, text width=180pt]]
                [General Benchmark, [{S-Eval \cite{yuan2024s}, BELLS \cite{dorn2024bells}, Agent-SafetyBench \cite{zhang2024safetybench}, Agent Security Bench \cite{zhang2024asb}, AgentHarm \cite{andriushchenko2024agentharm}, RJudge \cite{yuan2024r}}, answer_work, text width=180pt]]
            ]
        ]
        [Memory, for tree={
            answer,
            calign=child edge, calign child=(n_children()+1)/2,
            yshift=-0.2cm,
            }
            [Attack, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Memory Poisoning, [{RobustRAG \cite{xiang2024certifiably}, AgentPoison \cite{chen2025agentpoison}, PoisonedRAG \cite{zou2024poisonedrag}, Zhong et al. \cite{zhong2023poisoning}, Zhang et al. \cite{zhang2024agent}, Gu et al. \cite{gu2024agent}, GARAG \cite{cho2024typos}}, answer_work, text width=200pt, fill=white]]
                [Privacy Leakage, [{Li et al. \cite{li2025commercial}, Zeng et al. \cite{zeng2024good}, RAG-MIA \cite{anderson2024my}, RAG-Thief \cite{jiang2024rag}, Morris et al. \cite{morris2023text}, Li et al. \cite{li2023sentence}}, answer_work, text width=160pt]]
                [Memory Misuse, [{Russinovich et al. \cite{russinovich2024great}, li et al. \cite{li2024llm}, Cheng et al. \cite{cheng2024leveraging}, Priyanshu et al. \cite{priyanshu2024fractured}, Agarwal et al. \cite{agarwal2024prompt}, Tong et al. \cite{tong2024securing}}, answer_work, text width=180pt]]
            ]
            [Defense, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Detection, [{TrustRAG \cite{zhou2025trustrag}, Xian et al. \cite{xian2024vulnerability}, Agarwal et al. \cite{agarwal2024prompt}, ASB \cite{zhang2024agent}, MemoAnalyizer \cite{zhang2024ghost}}, answer_work, text width=270pt]]
                [Prompt Modification, [{Anderson et al. \cite{anderson2024my}, Agarwal et al. \cite{agarwal2024prompt}}, answer_work, text width=120pt]]
                [Output Intervention, [{RobustRAG \cite{xiang2024certifiably}, Chen et al. \cite{chen2023understanding}}, answer_work, text width=110pt]]]
            [Evaluation, [{PoisonedRAG \cite{zou2024poisonedrag}, AgentPoison \cite{chen2025agentpoison}, Zeng et al. \cite{zeng2024good}, RAG-Thief \cite{jiang2024rag}}, answer_work, text width=220pt]]
        ]
        [Tool, for tree={
            answer,
            calign=child edge, calign child=(n_children()+1)/2,
            yshift=-0.2cm,
            }
            [Attack, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Tool Manipulation, [{Cheng et al. \cite{cheng2024security}, Imprompter \cite{fu2024imprompter}, Fu et al. \cite{fu2023misusing}, BreakingAgents \cite{zhang2024breaking}, ToolCommander \cite{wang2024allies}, AUTOCMD \cite{jiang2025mimicking}, Zhao et al. \cite{zhao2024attacks}}, answer_work, text width=200pt]]
                [Tool Abuse, [{Fang et al. \cite{fang2024llm}, BadAgent \cite{wang2024badagent}, Kumar et.al \cite{kumar2024refusal}, Fang et al. \cite{fang2024llm}}, answer_work, text width=200pt]]
            ]
            [Defense, [{GuardAgent \cite{xiang2024guardagent}, AgentGuard \cite{chen2025agentguard}}, answer_work, text width=120pt]]
            [Evaluation, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Dataset Testing, [{ToolSword \cite{ye2024toolsword}, InjectAgent \cite{zhan2024injecagent}, AgentHarm \cite{andriushchenko2024agentharm}, PrivacyLens \cite{shao2025privacylens}}, answer_work, text width=220pt]]
                [Sandbox Simulation, [{ToolEmu \cite{ruan2023identifying}, HAICosystem \cite{zhou2024haicosystem}}, answer_work, text width=120pt]]
            ]
        ]
    ]
    [Extrinsic Trustworthiness, for tree={
        answer,
        calign=child edge, calign child=(n_children()+1)/2,
        yshift=-0.2cm,
        }
        [Agent, for tree={
            answer,
            calign=child edge, calign child=(n_children()+1)/2,
            yshift=-0.2cm,
            }
            [Attack, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Cooperative Attack, [{Ju et al. \cite{ju2024flooding}, Agent-in-the-Middle \cite{he2025red}, Amayuelas et al. \cite{amayuelas2024multiagent}, Eval Geniuses \cite{tian2023evil}}, answer_work, text width=260pt]]
                [Infectious Attack, [{Prompt Infection \cite{lee2024prompt}, CORBA \cite{zhou2025corba}, AgentSmith \cite{gu2024agent}, Tan et al. \cite{tan2024wolf}, NetSafe \cite{yu2024netsafe}}, answer_work, text width=270pt]]
            ]
            [Defense, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Cooperative Defense, [{BlockAgents \cite{chen2024blockagents}, Audit-LLM \cite{song2024audit}, chern et al. \cite{chern2024combating}, AutoDefense \cite{zeng2024autodefense}, LLAMOS \cite{lin2024large}, PsySafe \cite{zhang2024psysafe}}, answer_work, text width=170pt]]
                [Topological Defense, [{GPTSwarm \cite{zhuge2024gptswarm}, G-Safeguard \cite{wang2025g}}, answer_work, text width=120pt]]
            ]
            [Evaluation, [{SafeAgentBench \cite{yin2024safeagentbench}, R-judge \cite{yuan2024r}, JAILJUDGE \cite{benchmarkjailjudge}}, answer_work, text width=180pt, fill=white]
            ]
        ]
        [Environment, for tree={
            answer,
            calign=child edge, calign child=(n_children()+1)/2,
            yshift=-0.2cm,
            }
            [Physical Environment, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Robotics, [{Yang et al. \cite{yang2024plug}, SELP \cite{wu2024selp}}, answer_work, text width=110pt]]
                [Autonomous Driving, [{Hudson \cite{song2024enhancing}, ChatScene \cite{zhang2024chatscene}}, answer_work, text width=110pt]]
                [Industrial Control, [{Vyas et al. \cite{vyas2024autonomous}, Agents4PLC \cite{liu2024agents4plc}}, answer_work, text width=120pt]]
            ]
            [Digital Environment, for tree={
                answer,
                calign=child edge, calign child=(n_children()+1)/2,
                yshift=-0.2cm,
                }
                [Network, [{Fang et al. \cite{fang2024llm}, Debenedetti et al. \cite{debenedetti2024agentdojo}}, answer_work, text width=130pt]]
                [Healthcare, [{Xiang et al. \cite{xiang2024guardagent}, Polaris \cite{mukherjee2024polaris}}, answer_work, text width=110pt]]
                [Finance, [{Chen et al. \cite{chen2025position}, Park et al. \cite{park2024enhancing}}, answer_work, text width=110pt]]
                [Social Media, [{Jeptoo et al. \cite{jeptoo2024enhancing}, La et al. \cite{la2024safeguarding}}, answer_work, text width=110pt]]
            ]
        ]
        [User, [{He et al. \cite{he2024emerged}, Zhang et al. \cite{zhang2024privacy}, Sun et al. \cite{sun2024empowering}}, answer_work, text width=160pt, fill=white]]
    ]
]
]
\end{forest}
\caption{A comprehensive taxonomy of TrustAgent, categorized according to agent modules.}
\end{figure*}
